RealChart2Code: Advancing Chart-to-Code Generation with Real Data and Multi-Task Evaluation

Vision-Language Models (VLMs) have demonstrated impressive capabilities in code generation across various domains. However, their ability to replicate complex, multi-panel visualizations from real-world data remains largely unassessed. To address this gap, we introduce \textbf{\texttt{RealChart2Code}}, a new large-scale benchmark with over 2,800 instances grounded in authentic datasets and featuring tasks with clear analytical intent. Crucially, it is the first benchmark to systematically evaluate chart generation from large-scale raw data and assess iterative code refinement in a multi-turn conversational setting. Our comprehensive evaluation of 14 leading VLMs on \texttt{RealChart2Code} reveals significant performance degradation compared to simpler benchmarks, highlighting their struggles with complex plot structures and authentic data. Our analysis uncovers a substantial performance gap between proprietary and open-weight models and confirms that even state-of-the-art VLMs often fail to accurately replicate intricate, multi-panel charts. These findings provide valuable insights into the current limitations of VLMs and guide future research directions. We release the benchmark and code at \url{https://github.com/Speakn0w/RealChart2Code}.

==> latex/tables/benchmarks_table.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of \textbf{RealChart2Code} with existing chart-to-code benchmarks. A \cmark indicates the presence of a feature, while a \xmark indicates its absence.}
\label{tab:benchmark-comparison}
\small
\begin{tabular}{l cccc}
\toprule
\textbf{Benchmark} & \textbf{\# of Test Instances} & \textbf{Real-World Data} & \textbf{Complex Charts} & \textbf{Multi-Turn Dialogue} \\
\midrule
Plot2Code~\citep{plot2code}   & 132   & \xmark & \xmark & \xmark \\
Design2Code~\citep{si2024design2code}& 484 & \xmark & \xmark & \xmark \\
ChartMimic \citep{chartmimic}  & 4800   & \xmark & \xmark & \xmark \\
\rowcolor{gray!15}
\textbf{RealChart2Code} (Ours) & 2874 & \cmark & \cmark & \cmark \\
\bottomrule
\end{tabular}
\end{table*}

